LiDAR ICPS-net: Indoor Camera Positioning based-on Generative Adversarial Network for RGB to Point-Cloud Translation

Indoor positioning aims at navigation inside areas with no GPS-data availability and could be employed in many applications such as augmented reality, autonomous driving specially inside closed areas and tunnels. In this paper, a deep neural network-based architecture has been proposed to address this problem. In this regard, a tandem set of convolutional neural networks, as well as a Pix2Pix GAN network have been leveraged to perform as the scene classifier, scene RGB image to point cloud converter, and position regressor, respectively. The proposed architecture outperforms the previous works, including our recent work, in the sense that it makes data generation task easier and more robust against scene small variations, whilst the accuracy of the positioning is remarkably well, for both Cartesian position and quaternion information of the camera.

==> urlbst <==
#! /usr/bin/perl -w
#
# Usage: ./urlbst.pl [--eprint] [--doi] [--pubmed]
#    [--nohyperlinks] [--inlinelinks] [--hypertex] [--hyperref]
#    [input-file [output-file]]
# If either input-file or output-file is omitted, they are replaced by
# stdin or stdout respectively.
#
# See http://purl.org/nxg/dist/urlbst for documentation
#
# Copyright 2002-03, 2005-12, 2014, 2019, Norman Gray <http://nxg.me.uk>
#
# This program is distributed under the terms of the
# GNU General Public Licence, v2.0.
# The modifications to the input .bst files are asserted as Copyright 2002-03, 2005-12, 2014, 2019, Norman Gray,
# and distributed under the terms of the LaTeX Project Public Licence.
# See the package README for further dicussion of licences.

$version = '0.8';
($progname = $0) =~ s/.*\///;
$mymarker = "% $progname";
$mymarkerend = "% ...$progname to here";
$myurl = 'http://purl.org/nxg/dist/urlbst';


$infile = '-';
$outfile = '-';

$addeprints = 1;     # if true (nonzero) we add support for eprints
$literals{eprintprefix} = 'arXiv:';	# make these settable with --eprint? syntax?
$eprinturl = 'http://arxiv.org/abs/';

$adddoiresolver = 1;
$literals{doiprefix} = 'doi:';
$doiurl = 'https://doi.org/';

$addpubmedresolver = 1;
$literals{pubmedprefix} = 'PMID:';
$pubmedurl = 'http://www.ncbi.nlm.nih.gov/pubmed/';

$makehref = 0;
$literals{urlintro} = "URL: ";
$inlinelinks = 0;

$literals{online} = "online";
$literals{cited} = "cited ";
$literals{linktext} = "[link]";

$automatic_output_filename = 0;

$Usage = "$progname [--eprint] [--doi] [--pubmed]\n    [--nohyperlinks] [--[no]inlinelinks] [--hypertex] [--hyperref]\n    [--literal key=value]\n    [--help] [input-file [output-file]]";

# Magic environment variable: if this is set, then we're being called from a Platypus wrapper
# See http://www.sveinbjorn.org/platypus
if ($ENV{"CALLED_FROM_PLATYPUS"}) {
    $automatic_output_filename = 1;
}

while ($#ARGV >= 0) {
    if ($ARGV[0] eq '--eprint') {
	$addeprints = 1;
    } elsif ($ARGV[0] eq '--noeprint') {
	$addeprints = 0;
    } elsif ($ARGV[0] eq '--doi') {
        $adddoiresolver = 1;
    } elsif ($ARGV[0] eq '--nodoi') {
        $adddoiresolver = 0;
    } elsif ($ARGV[0] eq '--pubmed') {
        $addpubmedresolver = 1;
    } elsif ($ARGV[0] eq '--nopubmed') {
        $addpubmedresolver = 0;
    } elsif ($ARGV[0] eq '--nohyperlinks') {
        $makehref = 0;
    } elsif ($ARGV[0] eq '--hypertex') {
	$makehref = 1;
    } elsif ($ARGV[0] eq '--hyperref') {
	$makehref = 2;
    } elsif ($ARGV[0] eq '--inlinelinks') {
        $inlinelinks = 1;
    } elsif ($ARGV[0] eq '--noinlinelinks') {
        $inlinelinks = 0;
    } elsif ($ARGV[0] eq '--automatic-output') {
        $automatic_output_filename = 1;
    } elsif ($ARGV[0] eq '--literal') {
        shift;
        my $showstrings = 0;
        if ((($k, $v) = ($ARGV[0] =~ /^(\w+)=(.*)/)) && exists $literals{$k}) {
            $literals{$k} = $v;
        } elsif ($ARGV[0] eq 'help') {
            $showstrings = 1;
        } else {
            print "No literal found in $ARGV[0]; ignoring that\n";
            $showstrings = 1;
        }
        if ($showstrings) {
            print "    Possible literal strings (and defaults) are...\n";
            while (($k, $v) = each (%literals)) {
                print "        $k ($v)\n";
            }
            exit(0);
        }
    } elsif ($ARGV[0] eq '--help') {
        print <<EOD;
urlbst version $version
    Usage: $Usage
      --[no]eprint        include support for `eprint' fields
      --[no]doi           include support for `doi' field
      --[no]pubmed        include support for `pubmed' field
      --nohyperlinks      do not include active links anywhere
      --[no]inlinelinks   add hyperlinks to entry titles
      --hypertex          include HyperTeX-style hyperlink support
      --hyperref          include {hyperref}-style hyperlink support
                          (generally better)
      --literal key=value set one of the literal strings
                          (see `--literal help' for possibilities)
      --help              print this help
    Input and output files may be given as `-' (default) to indicate stdin/out.

EOD
        printf("    Defaults:\n");
        printf("      eprint refs    %s\n", ($addeprints ? "included" : "not included"));
        printf("      DOIs           %s\n", ($adddoiresolver ? "included" : "not included"));
        printf("      PUBMED refs    %s\n", ($addpubmedresolver ? "included" : "not included"));
        printf("      hyperlinks     %s\n", ($makehref==0 ? "none" : $makehref==1 ? "hypertex" : "hyperref"));
        printf("      inline links   %s\n", ($inlinelinks ? "included" : "not included"));
        exit(0);
    } elsif ($ARGV[0] =~ /^-/) {
        die "Unrecognised option $ARGV[0]: Usage: $Usage\n";
    } elsif ($infile eq '-') {
	$infile = $ARGV[0];
    } elsif ($outfile eq '-') {
	$outfile = $ARGV[0];
    } else {
	die "Usage: $Usage\n";
    }
    shift(@ARGV);
}

if ($inlinelinks && $makehref == 0) {
    print <<'EOD';
Warning: --inlinelinks and --nohyperlinks were both specified (possibly
    implicitly).  That combination makes no sense, so I'll ignore
    --nohyperlinks and use --hyperref instead
EOD
    $makehref = 2;
}

if ($automatic_output_filename) {
    if ($infile eq '-') {
        print "ERROR: No input filename given with --automatic-output\n";
    }
    $outfile = $infile;
    @outparts = split /\./, $outfile;
    $ext = pop(@outparts);
    $outfile=join('.', @outparts);
    if ($outfile eq '') {
        $outfile = $ext . '-url';
    } else {
        $outfile = $outfile . '-url.' . $ext;
    }
}

$exitstatus = 0;		# success status

open (IN, "<$infile") || die "Can't open $infile to read";
open (OUT, ">$outfile") || die "Can't open $outfile to write";

# We have to make certain assumptions about the source files, in order
# to patch them at the correct places.  Specifically, we assume that
#
#   - there's a function init.state.consts
#
#   - ...and an output.nonnull which does the actual outputting, which
#         has the `usual' interface.
#
#   - we can replace
#           fin.entry
#       by
#           new.block
#           output.url    % the function which formats and displays any URL
#           fin.entry
#
#   - there is a function which handles the `article' entry type (this
#         will always be true)
#
#   - there is a function output.bibitem which is called at the
#         beginning of each entry type
#   - ...and one called fin.entry which is called at the end
#
# If the functions format.date, format.title or new.block are not defined (the
# former is not in apalike, for example, and the last is not in the
# AMS styles), then replacements are included in the output.
#
# All these assumptions are true of the standard files and, since most
# style files derive from them more or less directly, are true of most (?)
# other style files, too.
#
# There's some rather ugly Perl down here.  The parsing for
# brace-matching could probably do with being rewritten in places, to
# make it less ugly, and more robust.

print OUT "%%% Modification of BibTeX style file ", ($infile eq '-' ? '<stdin>' : $infile), "\n";
print OUT "%%% ... by $progname, version $version (marked with \"$mymarker\")\n%%% See <$myurl>\n";
print OUT "%%% Modifications Copyright 2002-03, 2005-12, 2014, 2019, Norman Gray,\n";
print OUT "%%% and distributed under the terms of the LPPL; see README for discussion.\n";
print OUT "%%%\n";
print OUT "%%% Added webpage entry type, and url and lastchecked fields.\n";
print OUT "%%% Added eprint support.\n"   if ($addeprints);
print OUT "%%% Added DOI support.\n"      if ($adddoiresolver);
print OUT "%%% Added PUBMED support.\n"   if ($addpubmedresolver);
print OUT "%%% Added HyperTeX support.\n" if ($makehref == 1);
print OUT "%%% Added hyperref support.\n" if ($makehref == 2);
print OUT "%%% Original headers follow...\n\n";

$found{initconsts} = 0;
$found{outputnonnull} = 0;
$found{article} = 0;
$found{outputbibitem} = 0;
$found{finentry} = 0;
$found{formatdate} = 0;
$found{formattitle} = 0;
$found{newblock} = 0;
# The following are initialised negative, which Perl treats as true,
# so the simple test 'if ($found{formateprint}) ...' will be true.
$found{formateprint} = -1;
$found{formatdoi} = -1;
$found{formatpubmed} = -1;

while (<IN>) {
    /^ *%/ && do {
        # Pass commented lines unchanged
        print OUT;
        next;
    };
    
    /^ *ENTRY/ && do {
	# Work through the list of entry types, finding what ones are there.
	# If we find a URL entry there already, object, since these edits
	# will mess things up.
	$line = $_;
	until ($line =~ /\{\s*(\w*)/) {
	    $line .= <IN>;
	}
	$bracematchtotal = 0;	# reset
	bracematcher($line);
	$line =~ /\{\s*(\w*)/;
	$found{'entry'.$1} = 1;
	print OUT $line;
	$line = <IN>;
	until (bracematcher($line) == 0) {
	    # XXX deal with multiple entries on one line
	    ($line =~ /^\s*(\w*)/) && ($found{'entry'.$1} = 1);
	    print OUT $line;
	    $line = <IN>;
	}
	if (defined($found{entryurl})) {
	    print STDERR "$progname: style file $infile already has URL entry!\n";
	    # print out the rest of the file, and give up
            print OUT $line;
	    while (<IN>) {
		print OUT;
	    }
	    $exitstatus = 1;
	    last;
	} else {
            print OUT "    eprint $mymarker\n    doi $mymarker\n    pubmed $mymarker\n    url $mymarker\n    lastchecked $mymarker\n";
	}
	print OUT $line;
	next;
    };

    /^ *FUNCTION *\{init\.state\.consts\}/ && do {
        # In the init.state.consts function, add an extra set of
        # constants at the beginning.  Also use this as the marker for
        # the place to add the init strings function.
        print OUT <<EOD;
$mymarker...
% urlbst constants and state variables
STRINGS { urlintro
  eprinturl eprintprefix doiprefix doiurl pubmedprefix pubmedurl
  citedstring onlinestring linktextstring
  openinlinelink closeinlinelink }
INTEGERS { hrefform inlinelinks makeinlinelink
  addeprints adddoiresolver addpubmedresolver }
FUNCTION {init.urlbst.variables}
{
  % The following constants may be adjusted by hand, if desired

  % The first set allow you to enable or disable certain functionality.
  #$addeprints 'addeprints :=         % 0=no eprints; 1=include eprints
  #$adddoiresolver 'adddoiresolver :=     % 0=no DOI resolver; 1=include it
  #$addpubmedresolver 'addpubmedresolver :=     % 0=no PUBMED resolver; 1=include it
  #$makehref 'hrefform :=           % 0=no crossrefs; 1=hypertex xrefs; 2=hyperref refs
  #$inlinelinks 'inlinelinks :=        % 0=URLs explicit; 1=URLs attached to titles

  % String constants, which you _might_ want to tweak.
  "$literals{urlintro}" 'urlintro := % prefix before URL; typically "Available from:" or "URL":
  "$literals{online}" 'onlinestring := % indication that resource is online; typically "online"
  "$literals{cited}" 'citedstring := % indicator of citation date; typically "cited "
  "$literals{linktext}" 'linktextstring := % dummy link text; typically "[link]"
  "$eprinturl" 'eprinturl := % prefix to make URL from eprint ref
  "$literals{eprintprefix}" 'eprintprefix := % text prefix printed before eprint ref; typically "arXiv:"
  "$doiurl" 'doiurl := % prefix to make URL from DOI
  "$literals{doiprefix}" 'doiprefix :=      % text prefix printed before DOI ref; typically "doi:"
  "$pubmedurl" 'pubmedurl := % prefix to make URL from PUBMED
  "$literals{pubmedprefix}" 'pubmedprefix :=      % text prefix printed before PUBMED ref; typically "PMID:"

  % The following are internal state variables, not configuration constants,
  % so they shouldn't be fiddled with.
  #0 'makeinlinelink :=     % state variable managed by possibly.setup.inlinelink
  "" 'openinlinelink :=     % ditto
  "" 'closeinlinelink :=    % ditto
}
INTEGERS { 
  bracket.state
  outside.brackets
  open.brackets
  within.brackets
  close.brackets
}
$mymarkerend
EOD
	$line = $_;
	until ($line =~ /\{.*\}.*\{/s) {
	    $line .= <IN>;
	}
	$line =~ s/(\{.*?\}.*?\{)/$1 #0 'outside.brackets := $mymarker...
  #1 'open.brackets :=
  #2 'within.brackets :=
  #3 'close.brackets := $mymarkerend

 /s;
	print OUT $line;
	$found{initconsts} = 1;
	next;
    };

    /^ *EXECUTE *\{init\.state\.consts\}/ && do {
        print OUT "EXECUTE {init.urlbst.variables} $mymarker\n";
        print OUT;
        next;
    };

    /^ *FUNCTION *\{new.block\}/ && do {
        $found{newblock} = 1;
    };

    /^ *FUNCTION *\{format.doi\}/ && do {
        #print STDERR "$progname: style file $infile already supports DOIs; urlbst format.doi disabled\n(see generated .bst style: you may need to make edits near \$adddoiresolver)\n";
        $found{formatdoi} = 1;
        $adddoiresolver = 0;
    };

    /^ *FUNCTION *\{format.eprint\}/ && do {
        #print STDERR "$progname: style file $infile already supports eprints; urlbst format.eprint disabled\n(see generated .bst style: you may need to make edits near \$addeprints)\n";
        $found{formateprint} = 1;
        $addeprints = 0;
    };

    /^ *FUNCTION *\{format.pubmed\}/ && do {
        #print STDERR "$progname: style file $infile already supports Pubmed; urlbst format.pubmed disabled\n(see generated .bst style: you may need to make edits near \$addpubmedresolver)\n";
        $found{formatpubmed} = 1;
        $addpubmedresolver = 0;
    };

    /^ *FUNCTION *{output\.nonnull}/ && do {
	print OUT "$mymarker\n";
	print OUT "FUNCTION {output.nonnull.original}\n";
        copy_block();
	print_output_functions();
	$found{outputnonnull} = 1;
	next;
    };

    /FUNCTION *\{fin.entry\}/ && do {
        # Rename fin.entry to fin.entry.original (wrapped below)
        s/fin.entry/fin.entry.original/;
        s/$/ $mymarker (renamed from fin.entry, so it can be wrapped below)/;
        $found{finentry} = 1;
        print OUT;
        next;
    };

    /^ *FUNCTION *{format\.date}/ && do {
	$found{formatdate} = 1;
	print OUT;
	next;
    };

    /^ *FUNCTION *{format\.title}/ && do {
        # record that we found this
	$found{formattitle} = 1;
        print OUT;
	next;
    };

    /^ *format\.b?title/ && do {
        # interpolate a call to possibly.setup.inlinelink
        print OUT "  title empty\$ 'skip\$ 'possibly.setup\.inlinelink if\$ $mymarker\n";
        print OUT;
        next;
    };

    /^ *format\.vol\.num\.pages/ && do {
        # interpolate a call to possibly.setup.inlinelink
        s/^( *)/$1possibly.setup.inlinelink /;
        s/$/$mymarker/;
        print OUT;
        next;
    };

    /^ *FUNCTION *\{article\}/ && do {

	print_missing_functions();
	print_webpage_def();

	print OUT;
	$found{article} = 1;
	next;
    };

    /FUNCTION *\{output.bibitem\}/ && do {
        # Rename output.bibitem to output.bibitem.original (wrapped below)
        s/{output.bibitem\}/\{output.bibitem.original\}/;
        s/$/ $mymarker (renamed from output.bibitem, so it can be wrapped below)/;
 	$found{outputbibitem} = 1;
        print OUT;
        next;
    };

    print OUT;
};

if ($exitstatus == 0) {
    # Skip this if we've already reported an error -- it'll only be confusing
    foreach $k (keys %found) {
        if ($found{$k} == 0) {
            print STDERR "$progname: $infile: failed to find feature $k\n";
        }
    }
}

close (IN);
close (OUT);

exit $exitstatus;;






sub print_output_functions {
    print OUT "$mymarker...\n";

    print OUT <<'EOD';
% The following three functions are for handling inlinelink.  They wrap
% a block of text which is potentially output with write$ by multiple
% other functions, so we don't know the content a priori.
% They communicate between each other using the variables makeinlinelink
% (which is true if a link should be made), and closeinlinelink (which holds
% the string which should close any current link.  They can be called
% at any time, but start.inlinelink will be a no-op unless something has
% previously set makeinlinelink true, and the two ...end.inlinelink functions
% will only do their stuff if start.inlinelink has previously set
% closeinlinelink to be non-empty.
% (thanks to 'ijvm' for suggested code here)
FUNCTION {uand}
{ 'skip$ { pop$ #0 } if$ } % 'and' (which isn't defined at this point in the file)
FUNCTION {possibly.setup.inlinelink}
{ makeinlinelink hrefform #0 > uand
    { doi empty$ adddoiresolver uand
        { pubmed empty$ addpubmedresolver uand
            { eprint empty$ addeprints uand
                { url empty$
                    { "" }
                    { url }
                  if$ }
                { eprinturl eprint * }
              if$ }
            { pubmedurl pubmed * }
          if$ }
        { doiurl doi * }
      if$
      % an appropriately-formatted URL is now on the stack
      hrefform #1 = % hypertex
        { "\special {html:<a href=" quote$ * swap$ * quote$ * "> }{" * 'openinlinelink :=
          "\special {html:</a>}" 'closeinlinelink := }
        { "\href {" swap$ * "} {" * 'openinlinelink := % hrefform=#2 -- hyperref
          % the space between "} {" matters: a URL of just the right length can cause "\% newline em"
          "}" 'closeinlinelink := }
      if$
      #0 'makeinlinelink :=
      }
    'skip$
  if$ % makeinlinelink
}
FUNCTION {add.inlinelink}
{ openinlinelink empty$
    'skip$
    { openinlinelink swap$ * closeinlinelink *
      "" 'openinlinelink :=
      }
  if$
}
EOD

    # new.block is defined elsewhere

    print OUT <<'EOD';
FUNCTION {output.nonnull}
{ % Save the thing we've been asked to output
  's :=
  % If the bracket-state is close.brackets, then add a close-bracket to
  % what is currently at the top of the stack, and set bracket.state
  % to outside.brackets
  bracket.state close.brackets =
    { "]" *
      outside.brackets 'bracket.state :=
    }
    'skip$
  if$
  bracket.state outside.brackets =
    { % We're outside all brackets -- this is the normal situation.
      % Write out what's currently at the top of the stack, using the
      % original output.nonnull function.
      s
      add.inlinelink
      output.nonnull.original % invoke the original output.nonnull
    }
    { % Still in brackets.  Add open-bracket or (continuation) comma, add the
      % new text (in s) to the top of the stack, and move to the close-brackets
      % state, ready for next time (unless inbrackets resets it).  If we come
      % into this branch, then output.state is carefully undisturbed.
      bracket.state open.brackets =
        { " [" * }
        { ", " * } % bracket.state will be within.brackets
      if$ 
      s * 
      close.brackets 'bracket.state :=
    }
  if$
}

% Call this function just before adding something which should be presented in 
% brackets.  bracket.state is handled specially within output.nonnull.
FUNCTION {inbrackets}
{ bracket.state close.brackets =
    { within.brackets 'bracket.state := } % reset the state: not open nor closed
    { open.brackets 'bracket.state := }
  if$
}

FUNCTION {format.lastchecked}
{ lastchecked empty$
    { "" }
    { inbrackets citedstring lastchecked * }
  if$
}
EOD
    print OUT "$mymarkerend\n";
}

sub print_webpage_def {
    print OUT "$mymarker...\n";

    # Some of the functions below call new.block, so we need a dummy
    # version, in the case where the style being edited doesn't supply
    # that function.
    if (! $found{newblock}) {
        print OUT "FUNCTION {new.block} % dummy new.block function\n{\n  % empty\n}\n\n";
        $found{newblock} = 1;
    }

    print OUT <<'EOD';
% Functions for making hypertext links.
% In all cases, the stack has (link-text href-url)
%
% make 'null' specials
FUNCTION {make.href.null}
{
  pop$
}
% make hypertex specials
FUNCTION {make.href.hypertex}
{ 
  "\special {html:<a href=" quote$ *
  swap$ * quote$ * "> }" * swap$ *
  "\special {html:</a>}" *
}
% make hyperref specials
FUNCTION {make.href.hyperref}
{ 
  "\href {" swap$ * "} {\path{" * swap$ * "}}" *
}
FUNCTION {make.href}
{ hrefform #2 =
    'make.href.hyperref      % hrefform = 2
    { hrefform #1 =
        'make.href.hypertex  % hrefform = 1
        'make.href.null      % hrefform = 0 (or anything else)
      if$
    }
  if$
}

% If inlinelinks is true, then format.url should be a no-op, since it's
% (a) redundant, and (b) could end up as a link-within-a-link.
FUNCTION {format.url}
{ inlinelinks #1 = url empty$ or
   { "" }
   { hrefform #1 =
       { % special case -- add HyperTeX specials
         urlintro "\url{" url * "}" * url make.href.hypertex * }
       { urlintro "\url{" * url * "}" * }
     if$
   }
  if$
}
EOD

    $formateprintfunction = <<'EOD';
FUNCTION {format.eprint}
{ eprint empty$
    { "" }
    { eprintprefix eprint * eprinturl eprint * make.href }
  if$
}
EOD
    output_replacement_function($found{formateprint},
                                'format.eprint',
                                'addeprints',
                                $formateprintfunction);

    $formatdoifunction = <<'EOD';
FUNCTION {format.doi}
{ doi empty$
    { "" }
    { doiprefix doi * doiurl doi * make.href }
  if$
}
EOD
    output_replacement_function($found{formatdoi},
                                'format.doi',
                                'adddoiresolver',
                                $formatdoifunction);

    $formatpubmedfunction = <<'EOD';
FUNCTION {format.pubmed}
{ pubmed empty$
    { "" }
    { pubmedprefix pubmed * pubmedurl pubmed * make.href }
  if$
}
EOD
    output_replacement_function($found{formatpubmed},
                                'format.pubmed',
                                'addpubmedresolver',
                                $formatpubmedfunction);

    print OUT <<'EOD';
% Output a URL.  We can't use the more normal idiom (something like
% `format.url output'), because the `inbrackets' within
% format.lastchecked applies to everything between calls to `output',
% so that `format.url format.lastchecked * output' ends up with both
% the URL and the lastchecked in brackets.
FUNCTION {output.url}
{ url empty$
    'skip$ 
    { new.block 
      format.url output
      format.lastchecked output 
    }
  if$
}

FUNCTION {output.web.refs}
{
  new.block
  inlinelinks
    'skip$ % links were inline -- don't repeat them
    { % If the generated DOI will be the same as the URL,
      % then don't print the URL (thanks to Joseph Wright for this code,
      % at http://tex.stackexchange.com/questions/5660)
      adddoiresolver 
          doiurl doi empty$ { "X" } { doi } if$ * % DOI URL to be generated
          url empty$ { "Y" } { url } if$          % the URL, or "Y" if empty
          =                                       % are the strings equal?
          and
        'skip$
        { output.url }
      if$
      addeprints eprint empty$ not and
        { format.eprint output.nonnull }
        'skip$
      if$
      adddoiresolver doi empty$ not and
        { format.doi output.nonnull }
        'skip$
      if$
      addpubmedresolver pubmed empty$ not and
        { format.pubmed output.nonnull }
        'skip$
      if$
    }
  if$
}

% Wrapper for output.bibitem.original.
% If the URL field is not empty, set makeinlinelink to be true,
% so that an inline link will be started at the next opportunity
FUNCTION {output.bibitem}
{ outside.brackets 'bracket.state :=
  output.bibitem.original
  inlinelinks url empty$ not doi empty$ not or pubmed empty$ not or eprint empty$ not or and
    { #1 'makeinlinelink := }
    { #0 'makeinlinelink := }
  if$
}

% Wrapper for fin.entry.original
FUNCTION {fin.entry}
{ output.web.refs  % urlbst
  makeinlinelink       % ooops, it appears we didn't have a title for inlinelink
    { possibly.setup.inlinelink % add some artificial link text here, as a fallback
      linktextstring output.nonnull }
    'skip$
  if$
  bracket.state close.brackets = % urlbst
    { "]" * }
    'skip$
  if$
  fin.entry.original
}

% Webpage entry type.
% Title and url fields required;
% author, note, year, month, and lastchecked fields optional
% See references 
%   ISO 690-2 http://www.nlc-bnc.ca/iso/tc46sc9/standard/690-2e.htm
%   http://www.classroom.net/classroom/CitingNetResources.html
%   http://neal.ctstateu.edu/history/cite.html
%   http://www.cas.usf.edu/english/walker/mla.html
% for citation formats for web pages.
FUNCTION {webpage}
{ output.bibitem
  author empty$
    { editor empty$
        'skip$  % author and editor both optional
        { format.editors output.nonnull }
      if$
    }
    { editor empty$
        { format.authors output.nonnull }
        { "can't use both author and editor fields in " cite$ * warning$ }
      if$
    }
  if$
  new.block
  title empty$ 'skip$ 'possibly.setup.inlinelink if$
  format.title "title" output.check
  inbrackets onlinestring output
  new.block
  year empty$
    'skip$
    { format.date "year" output.check }
  if$
  % We don't need to output the URL details ('lastchecked' and 'url'),
  % because fin.entry does that for us, using output.web.refs.  The only
  % reason we would want to put them here is if we were to decide that
  % they should go in front of the rather miscellaneous information in 'note'.
  new.block
  note output
  fin.entry
}
EOD

    print OUT "$mymarkerend\n\n\n";
}


sub output_replacement_function {
    my $emit_function = $_[0];
    my $function_name = $_[1];
    my $disabling_variable = $_[2];
    my $function_definition_string = $_[3];

    if ($emit_function > 0) {
        print OUT <<"EOD";
%%% The style file $infile already supports $function_name,
%%% but it might not do so in the same way as urlbst expects.
%%% I've therefore left $infile 's function unchanged,
%%% and disabled urlbst's version; proceed with some caution.
EOD

        print STDERR "$progname: WARNING: style file $infile already includes a $function_name function;\nyou may need to disable the urlbst version by setting \$$disabling_variable to zero.\nYou might want to edit the output file (search for $function_name).\n";

        ($t = $function_definition_string) =~ s/\n/\n%%% /g;
        print OUT "%%% " . $t . "$mymarker\n";
    } else {
        print OUT $function_definition_string;
    }
    print OUT "\n";
}

sub print_missing_functions {
    # We've got to the bit of the file which handles the entry
    # types, so write out the webpage entry handler.  This uses
    # the format.date function, which which many but not all
    # bst files have (for example, apalike doesn't).  So
    # check that we either have found this function already, or
    # add it.
    if (! $found{formatdate}) {
	if ($found{entrymonth}) {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    { month empty$
	{ "" }
	{ "there's a month but no year in " cite$ * warning$
	  month
	}
      if$
    }
    { month empty$
	'year
	{ month " " * year * }
      if$
    }
  if$
}
EOD
	} else {
	    print OUT <<'EOD';
FUNCTION {format.date}
{ year empty$
    'skip$
    { %write$
      "(" year * ")" *
    }
  if$
}
EOD
  	}
	$found{formatdate} = 1;
    }

    # If the style file didn't supply a format.title function, then supply
    # one here (the {webpage} function requires it).
    if (! $found{formattitle}) {
	print OUT <<'EOD';
FUNCTION {format.title}
{ title empty$
    { "" }
    { title "t" change.case$ }
  if$
}
EOD
    $found{formattitle} = 1;
    }
}

# Utility function: Keep track of open and close braces in the string argument.
# Keep state in $bracematchtotal, return the current value.
sub bracematcher {
    my $s = shift;
    $s =~ s/[^\{\}]//g;
    #print "s=$s\n";
    foreach my $c (split (//, $s)) {
	$bracematchtotal += ($c eq '{' ? 1 : -1);
    }
    return $bracematchtotal;
}

# Utility function: use bracematcher to copy the complete block which starts
# on or after the current line.
sub copy_block {
    $bracematchtotal = 0;
    # copy any leading lines which don't have braces (presumably comments)
    while (defined ($line = <IN>) && ($line !~ /{/)) {
        print OUT $line;
    }
    while (defined ($line) && bracematcher($line) > 0) {
        print OUT $line;
        $line = <IN>;
    }
    print OUT "$line\n";	# print out terminating \} (assumed
    				# alone on the line)
}

